Antisite defects stabilized by antiphase boundaries in YFeO$_3$ thin films

YFeO$_3$ thin films are a recent addition to the family of multiferroic orthoferrites where Y\textsubscript{Fe} antisite defects and strain have been shown to introduce polar displacements while retaining magnetic properties. Complete control of the multiferroic properties, however, necessitates knowledge of the defects present and their potential role in modifying behavior. Here, we report the structure and chemistry of antiphase boundaries in multiferroic YFeO$_3$ thin films using aberration corrected scanning transmission electron microscopy combined with atomic resolution energy dispersive X-ray spectroscopy. We find that Fe\textsubscript{Y} antisites, which are not stable in the film bulk, periodically arrange along antiphase boundaries due to changes in the local environment. Using density functional theory, we show that the antiphase boundaries are polar and bi-stable, where the presence of Fe\textsubscript{Y} antisites significantly decreases the switching barrier. These results highlight how planar defects, such as antiphase boundaries, can stabilize point defects that would otherwise not be expected to form within the structure.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
